Generative Layout Modeling using Constraint Graphs

We propose a new generative model for layout generation. We generate layouts in three steps. First, we generate the layout elements as nodes in a layout graph. Second, we compute constraints between layout elements as edges in the layout graph. Third, we solve for the final layout using constrained optimization. For the first two steps, we build on recent transformer architectures. The layout optimization implements the constraints efficiently. We show three practical contributions compared to the state of the art: our work requires no user input, produces higher quality layouts, and enables many novel capabilities for conditional layout generation.

==> sections/models.tex <==
% As previously alluded to, our models use the Transformer \cite{vaswani2017transformers} as a building block. Our Element Constraint Model and the Edge model are very similar to the Vertex and Face models from PolyGen \cite{nash2020polygen} in roganization. The building block for the Transformers is based on the GPT-2 model, specifically, we use the GELU activation \cite{hendrycks2016gelu}, Layer Norm \cite{layernorm19} and dropout. For a complete description, please refer to the supplementary.

% The model for element constraint generation consists of 12 layers of our Transformers blocks. The sequence lengths depend on the particular dataset used, and are listed in the supplementary.

% The edge generation model is a Pointer Network with two-parts: 1. An encoder which generates embeddings, and can attend to all elements in the sequence of element constraints and 2. A decoder which generates pointers, and can attend to elements in an autoregressive fashion. In our experiments, use an encoder with 16 layers and a decoder with 12 layers. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{images/enc_dec_image.pdf}
%     \caption{The embedding generation model in the Pointer Network. Having an unmasked encoder allows our network to attend to all elements of the constraint sequence}
%     \label{fig:enc_dec_model}
% \end{figure}

% We perform constrained generation (Section \ref{sec:results}). This is performed by a variant of the edge generation model defined previously. Concretely, we change the encoder of Pointer Network to an encoder-decoder network $\hat{\mathbf{E}}-\hat{\mathbf{D}}$. The encoder $\hat{\mathbf{E}}$ is also a stack of Transformer blocks allowed to attend all elements of the sequence describing the constraints, and the decoder $\hat{\mathbf{D}}$ is another stack of blocks allowed to attend to all elements of the sequence constraints, and also performs cross-attention with the activations from $\hat{\mathbf{E}}$. We use 3 layers for $\hat{\mathbf{E}}$.

% We use 384 dimensional embeddings in all our models.

% \subsection{Training}
% We implemented our models in Pytorch\cite{paszke2017automatic}. Our models and sequences are small enough so we train on a single NVIDIA-V100 GPU with 32 GB memory. We use a constant learning-rate of $10^{-4}$, with a linear warmup for 500 iterations. The element generation model is trained for 40 epochs. The other models are trained for 80 epochs. It takes about 6 hours to train for our largest model for constrained generation.

==> source/sections/conclusion.tex <==
We proposed a new generative model for layout generation. Our model first generates a layout graph with layout elements as nodes and constraints between layout elements as edges. The final layout is computed by optimization. Our model overcomes many limitations of previous models, mainly the need for significant user input and ad-hoc post-processing steps. Further, our model leads to significantly higher generation quality as evidences by multiple statistics and enables multiple possibilities of conditional layout generation.
In future work, we would like to explore the application of our model to other layout problems, such as image layouts, 3D scene layouts, and component-based object modeling. We also would like to explore if our model can be used to post-process 3D scans of indoor environments. 

==> source/sections/introduction.tex <==
We study the problem of topologically and spatially consistent layout generation. This problem arises in image layout synthesis, floor plan synthesis, furniture layout generation, street layout planning, and part-based object creation, to name a few.
Generated content must meet stringent criteria both globally, in terms of its overall \textit{topological} structure, as well as locally, in terms of its \textit{spatial} detail.
While our work applies to layouts in general, we focus our discussion on two types of layouts: floorplans and furniture layouts.
%
%in the context of apartment floor plan and room-level furniture layouts. The proposed ideas can be extended to directly related 2D problems, such as street layout, graphic element layout on a page; as well as 3D problems involving part-based object creation or plant modeling.

% Example scenarios range from many variations of layout synthesis (e.g., street layouts, floor plan layouts, furniture layouts) to more specialized settings of part-based object creation, plant modeling, or chemical synthesis (i.e., layout of molecules).  Realism of such generated content is often assessed by comparing distributions of their \textit{global} and \textit{local} properties against those from real-world statistics.

When assessing layouts, we must consider the global structure which is largely topological in nature, such as connectivity between individual elements or inter-element hop distance.
We are also concerned with spatial detail, such as 
%In terms of
%local structure, we are also concerned with spatial character, in terms of
the geometric realization of the elements and their relative positioning, both local and non-local. Realism of such generated content is often assessed by comparing distributions of their properties, both topological and spatial, against those from real-world statistics.

% \textit{Global properties} deal with both topological and coarse spatial attributes of the scene parts. Various statistical properties relating to node valency, distibution of node types, graph distances, relative placement, etc.~have been proposed to characterize such global properties. \textit{Local properties}, in contrast, capture fine-scale geometric details such as the shape of the boundary between neighboring elements. For example, Figure~\ref{fig:motivation} shows typical global and local features for building  floor plans obtained from real-world layouts. 

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=\columnwidth]{sections/figures/teaser.pdf}
%     \caption{We present Dual Domain GAN, a method that generates layouts with realistic \emph{spatial} properties, like the room layout in these floor plans, and \emph{topological} properties, like the connectivity between rooms, shown as a graph in the insets. Many types of layouts, such as floor plans, require a generative model to reason about both topological and spatial properties.}
%     \label{fig:teaser_key}
% \end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/teaser_1.pdf}
    \caption{We present a method for layout generation. Our approach can generate multiple types of layouts, such as the floor plans in the top row, where rooms are colored by type, and furniture layouts in the bottom row, where furniture pieces are colored by type. Layouts are represented as graphs, where nodes correspond to layout elements and edges to relationships between elements. In the top row, nodes represent rooms (illustrated with room-type icons), and edges relate rooms connected by doors (dotted lines). Unlike previous methods, our method does not require any input guidance and generates higher-quality layouts.}
    \label{fig:teaser}
\end{figure}

Techniques for synthesizing realistic content have made rapid progress in recent years due to the emergence of generative adversarial networks (GANs)~\cite{Goodfellow2014GANs,Zhu2017CycleGAN,styleGan18,Wang:2018:AAAI:graphGAN}, variational autoencoders (VAEs)~\cite{kingma2013auto, vahdat2020NVAE}, flow models~\cite{rezende2015variational, yang2019pointflow, vahdat2020NVAE}, and autoregressive models~\cite{Chen2020GPTImage}. However, satisfying \textit{both} topological and spatial properties still remains an open challenge. 

%RPLAN~\cite{Wu_DeepLayout_2019}, Graph2Plan~\cite{Graph2Plan20}, and HouseGAN~\cite{housegan2020}.
%great initial
Recently, three  papers targeting this challenging problem in the floor plan setting were published~\cite{Wu_DeepLayout_2019, Graph2Plan20, housegan2020}. While these papers often produce good looking floor plans, they require several simplifications to to tackle this difficult problem:
%due to the difficult nature of the problem, these methods required several simplifications to achieve their results:
1) RPLAN~\cite{Wu_DeepLayout_2019} and Graph2Plan~\cite{Graph2Plan20} require the outline of the floorplan to be given.
2) HouseGAN~\cite{housegan2020} does not generate the connectivity between rooms that would be given by doors, and RPLAN places doors using a manually defined heuristic that is not learned from data.
3) HouseGAN and Graph2Plan require the number of rooms, the room types and their topology to be given as input in the form of an adjacency graph.
4) All three methods require a heuristic post-process that is essential to make the floorplan look more realistic, but that is not learned from data. In addition, there is still a lot of room to improve the quality and realism of the results.

In this paper, we would like to explore two ideas to improve upon this exciting initial work.
First, after extensive experiments with many variations of graph-based GANs and VAEs, we found that these architectures are not well suited
%that suitable
to tackle the problem. It is our conjecture that these methods struggle with the discrete nature of graphs and layouts.
%in general.
We therefore propose
%to use
an auto-regressive model using attention and self-attention layers. Such an architecture inherently handles discrete data and gives superior performance to current state of the art models. While transformer-based auto-regressive models~\cite{vaswani2017transformers} just started to compete with GANs built on CNNs in image generation~\cite{parmar2018image, chen2020generative} on the ImageNet~\cite{imagenet_cvpr09} dataset, the gap between these two competing approaches for \emph{layout generation} is significant.

Second, we explore the idea of generative modeling using constraint generation. We propose to model layouts with autoregressive models that generate constraint graphs: individual shapes are nodes and edges between nodes specify constraints.
%Node properties that satisfy the constraints are generated via optimization.
Our auto-regressive model first generates initial nodes, that are subsequently optimized to satisfy constraint edges generated by a second auto-regressive model.
%\paul{Check if both or only one model; depends how far we get with implementation}
These models can be conditioned on additional constraints provided by the user. This enables various forms of conditional generation and user interaction, from satisfying constraints provided by the user, to a fully generative model that generates constraints from scratch without user interaction.
%making it possible to have anything between a fully generative model that generates constraints from scratch, or .
For example, a user can optionally specify a floorplan boundary, or a set of rooms.
%Also, it is possible for the user to specify adjacency between a subset of the rooms.

% On the one hand, image-based generative methods produce impressive local geometric details, but struggle to generate content with the desired topological properties. On the other hand, the latest graph-based deep generative methods strive to match topological statistics to those of the training set but ignore spatial or geometric details.  Furthermore, the topological and spatial aspects are often coupled, as global layout constraints must respect local element shapes and alignments. %For example, Figure~\ref{fig:localGlobal} shows that image-only methods fail to match topological features in the  output. 

\if0
\begin{figure}[h!]
    \centering
    \includegraphics[width=\columnwidth]{sections/figures/localGlocalStats_motivation.pdf}
    \mycaption{Real versus generated layouts}
    {Image-based GANs (\textbf{Pix2Pix}, \textbf{StyleGAN}) produce layouts that spatially match real layouts, but poorly match topological statistics. In contrast, dual domain GAN (\textbf{DDGan}) matches both spatial and topological statistics. Here, `histogram of types of neighbors' as an example of topological statistics. See  Section~\ref{sec:results} for details. }
    \label{fig:localGlobal}
\end{figure}
\fi

% To address these challenges, we introduce \textit{dual domain GAN}  as the first deep generative framework to produce realistic layouts that match \textit{both} target topological attributes and spatial details. 
%
% In the first stage, \emph{spatial} properties are generated by a GAN in the image domain, this is followed by the second stage, in which \emph{topological} properties are generated by a GAN in the graph domain. The second stage is conditioned on the spatial properties generated in the first stage. Finally, we fuse the results from the two stages to produce layouts with both realistic spatial and topological features. 
%(Todo: add more information)


%To do so, we view the domain as an abstract graph, reflecting the connectivity among the elements, as well as an embedding of the elements encoding their geometric details.
%
%We capture both
%global and local
%properties using a novel data representation in the form of {\em embedded graphs} or \egraphs wherein, unlike regular graphs, the graph nodes additionally carry meaningful geometric embedding information. Such \egraphs capture both global topology or connectivity of the elements as well as spatial information relating to element attribute and layout (e.g., circular ordering of a node's neighbors, element size, placement). 

We demonstrate our approach in the context of floor plan generation by creating apartment-level room layouts and furniture layouts for each of the generated rooms (see Figure~\ref{fig:teaser}). Our evaluation will show that our generative model allows layout creation that matches both global and local statistics of real-world data much better than competing work. %Comparisons to image-only GANs are shown in Figure~\ref{fig:localGlobal}.


% maybe to discussion in the results section:
%Why not coarse-to-fine on a regular grid (images)?: Structures that are important for the topology, such as corridors, are not well captured by a low-res regular grid. The graph captures topology more explicitly (it captures exactly the relevant parts about topology, and allocates the same representation capacity to elements that are of similar importance to the topology) and thus makes the network reason about the topology.

%  We evaluate our method on two publicly available datasets, namely RPLAN~\cite{Wu_DeepLayout_2019} and LIFULL~\cite{lifull}, where our method achieves significant improvements in topological measures and spatial realism over state-of-the-art image-only and graph-only generation methods. We quantitatively evaluate the results of the dual domain GAN using common topological statistics, and qualitatively with a user study. In addition, we compare favorably against the state-of-the-art floor plan synthesis method~\cite{Wu_DeepLayout_2019}. 

In summary, we introduce two main contributions: 1) A transformer-based architecture for generative modeling of layouts that produces higher quality layouts than previous work. 2) The idea of a generative model that generates constraint graphs and solves for the spatial shape attributes via optimization, rather than outputting shapes directly.

==> source/sections/method.tex <==
%In this section, we first describe our input representation. We then describe how this input representation allows for a single architecture to handle different generation strategies with different levels of user-input. Finally, we present the full architecture and the training process.
%
% Our goal is to leverage powerful generative models
%

We present a generative model for layouts that can optionally be conditioned on constraints given by the user. Figure~\ref{fig:overview} illustrates our approach. Layouts are represented as graphs, where nodes correspond to discrete elements of the layout, and edges represent relationships between the elements.
%
We distinguish two types of edges: \emph{Constraining edges} describe desirable relationships between element parameters, such as an adjacency between a bedroom and a bathroom in a floor plan, and can be used to constrain these parameters. \emph{Descriptive edges} represent additional properties of the layout that are not given by the elements, but can be useful for down-stream tasks, such as the presence of a door between two rooms of a floor plan where the elements consist of rooms.
%
%We call the former \emph{constraining edges}, since they explicitly constrain relationships between element parameters, and the latter \emph{descriptive edges}, since they describe additional information that we cannot represent with the layout elements alone and that may be useful for down-stream tasks.
Section~\ref{sec:layout_rep} describes this layout representation.

%The user can provide constraints on both element parameters and both types of edges as input.

%Our model operates in two steps.

A generative model can be trained to generate both layout elements and edges. However, generated elements and generated constraining edges are not guaranteed to match. For example, two elements that are connected by an adjacency edge can often be separated by a gap, or can have overlaps. As the number of constraining edges increases, the problem of generating a compatible set of edges and elements becomes increasingly difficult to solve in a forward pass of the generative model. This has been a major limitation in previous work.

We introduce two contributions over previous layout generation methods. 
%
First, we show that a two-step autoregressive approach inspired by PolyGen~\cite{nash2020polygen} that first generates elements and then edges is particularly suitable for layout generation and performs significantly better than current methods. We describe this approach in Sections~\ref{sec:element_constraint_model} and~\ref{sec:edge_model}.

Second, we treat element parameters and constraining edges that were generated in the first two steps as \emph{constraints} and optimize element parameters to satisfy the generated constraints in a subsequent optimization step.
%
%allow for a larger range of user-provided constraints. Constraints can be specified on both element parameters and edges, and all constraints are optional: We can handle anything from layout generation without any user input, to providing a full layout graph as constraint. This is enabled by treating all element parameters and constraining edges that were generated in the first two steps as \emph{constraints}. We condition the generation of these constraints on the constraints provided by the user. This enables the user to provide constraints on an arbitrary subset of elements and/or edges of the layout.
%The generated constraints are used
%In a subsequent optimization step, we optimize element parameters to satisfy all generated constraints.  %adding a third step to our approach that optimizes elements to satisfy all user-provided constraints. We also treat all element parameters and constraining edges that were generated in the first two steps as \emph{constraints} for this optimization.
%
%we extend this two-step approach to allow for a larger range of user-provided constraints, by adding a third step to our approach that optimizes elements to satisfy the generated constraining edges, as well as edges provided by the user. We treat the generated element parameters and edges as \emph{constraints} for this optimization.
%training our approach to model the distribution of \emph{constraints} on element parameters and their relationships, instead of modelling the distribution of element parameters directly, and by adding a third step to our approach that optimizes elements to satisfy these generated constraints.
%
In floor plans, for example, we generate constraints on the maximum and minimum widths and heights of room areas and on their adjacency, and then solve for their locations, widths and heights in the optimization step.
%
This minimizes any discrepancies between constraining edges and element parameters.
%
%Note that without this optimization step, constraining edges cannot influence the generated elements, since edges are generated after elements.
%, and thus user-specified edge constraints would not be possible.
%
%Descriptive edges, on the other hand, are not needed to optimize element parameters and are generated in a separate step after the optimization.
%
%Thus, adding our optimization provides two main advantages: First, it enables us to handle user-provided edge constraints, such as constraints on the adjacency of layout elements. Second, our experiments show that the optimization allows us to satisfy constraints more accurately, especially as the number of constraints increases.
%
We describe the optimization in Section~\ref{sec:optimization}.
%
In Section~\ref{sec:user_constraints}, we describe how to condition on user-provided constraints.

%All generation steps are carefully conditioned on the user-provided constraints, to make the generated constraints as compatible as possible with the user-provided constraints. This conditioning is described in Section~\ref{sec:user_constraints}.

%Since edges are generated after elements, edges cannot influence element generation. This prevents us from including edge constraints provided by the user in the generation process. Additionally, this approach cannot guarantee that the generated relationships match the generated element parameters. For example, a generated adjacency edge could connect two elements that are not adjacent. As the number of constraint edges increases, the problem of generating a compatible set of edges and element parameters becomes increasingly difficult to solve in a forward pass of the generative model.
%
%Thus, our idea is to model the distribution of \emph{constraints} on element parameters and their relationships, instead of modelling the distribution of element parameters directly, and to add a third step to our approach that optimizes elements to satisfy these constraints. In floor plans, for example, we generate constraints on the widths and heights of room areas and on their adjacency, and solve for their locations in the optimization step. A description of the optimization is given in Section~\ref{sec:optimization}.

%In a first data-driven step, we use a Transformer-based model to generate constraints for element parameters and their relationships. We describe this step in Section~\ref{sec:constraint_generation}.
%
%In a second step, we optimize the full set of element parameters to match these constraints as closely as possible. This gives us a set of parameters that better match the constraints. A description of the optimization is given in Section~\ref{sec:optimization}.
%
%This two-step approach also makes it possible to include constraints provided by a user, as described in Section~\ref{sec:user_constraints}.

\subsection{Layout Representation}
\label{sec:layout_rep}

We represent layouts as a graph $\mathcal{L}=(\mathbf{N}, \mathbf{R})$, where nodes correspond to layout elements $\mathbf{N}$ and edges to their relationships $\mathbf{R}$. Each layout element $N \in \mathbf{N}$ has a fixed set of domain-specific parameters. Relationship edges $R \in \mathbf{R}$ are chosen from a fixed set of edge types $\rho$ and describe the presence of that edge between two elements $R = (N_i, N_j, \rho)$.
%
Edges come in two groups, based on their types: constraining edges $\mathbf{R}^C$ that provide constraints for the optimization step, and descriptive edges $\mathbf{R}^D$ that provide additional information about the layout.
%Some of the edge types are relationships that constrain element types $\mathbf{R}^C$ and relationships that add additional information to the layout $\mathbf{R}^L$, which are generated at different steps in our approach, as shown in Figure~\ref{fig:overview}.
%
We consider two main layout domains in our experiments: floor plans and furniture layouts, but will only focus on floor plans here. Furniture layouts are described in the supplementary material.
%Appendix~\ref{app:furniture}.

In floor plans, each layout element is a rectangular region of a room $N=(\tau, x,y,w,h)$, parameterized by the type of room $\tau$, the lower-left corner of the rectangular region $(x,y)$, and the width and height $(w,h)$ of the region. Two types of edges in $\mathbf{R}^C$ define horizontal and vertical adjacency constraints between elements, while two types of edges in $\mathbf{R}^D$, define the presence of a wall between two adjacent elements, and the presence of a door between two adjacent elements. Multiple elements of the same type that are adjacent and not separated by a wall form a room. The set of all elements fully cover the floor plan. An example is shown in Figure~\ref{fig:layout_examples}, left.
% \marginnote{Upper-left. Our origin is matrix style}[3cm]
%
More details on both representations, including a full list of all element types, are given in the supplementary material.
%Appendix~\ref{app:layout_rep}.

% \subsection{Constraint Generation}
% \label{sec:constraint_generation}

% We generate two types of layout constraints: constraints on the parameters of elements, and constraints on the relationships between element parameters. Inspired by PolyGen~\cite{nash2020polygen}, we employ two autoregressive sequence-to-sequence models to generate these constraints; a model based on transformers~\cite{vaswani2017transformers} for element constraints, and a model based on Pointer Networks~\cite{vinyals2015pointer} for relationship constraints.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/sequence_encoding.pdf}
    \caption{Example floor plan layout and its sequence encoding. Rooms are represented by rectangles, which are numbered and colored by room type for illustration (white for the exterior). Edges either constrain rectangles, like the red adjacency edges, or add information to the layout, like the blue door edges.
    %Doors are also illustrated by their architectural symbol.
    Both are encoded into sequences that can be ingested by our autoregressive sequence-to-sequence models.}
    \label{fig:layout_examples}
\end{figure}

\subsection{Element Constraint Model}
\label{sec:element_constraint_model}

An element constraint $N^C$ is defined as a tuple of target values for one or more of the parameters of element $N$. In the optimization, we will use these values as soft constraints for the corresponding parameters. We create one set of constraints for each element $N$ of the layout. In floor plans, for example, we create constraints $N^C = (\tau, w, h)$ for the type, width, and height of each element. All continuous values are treated as range constraints, i.e. the actual values may be within the range $\pm \epsilon v^C$ of the constraint value $v^C$ (we set $\epsilon=0.1$ in our experiments).
We use a transformer-based~\cite{vaswani2017transformers} autoregressive sequence-to-sequence model to generate these element constraints.

\paragraph{Sequence encoding}
The goal of our element constraint model is to learn a distribution over constraint sequences. To flatten our list of element constraints, we order them from left to right first (small to large $x$) and top to bottom (small to large $y$) for elements with the same $x$ coordinate. The ordered constraint tuples are concatenated to get a sequence of constraint values $S_E = (v_i)_{i=1}^{k M_N}$, where $M_N$ is the number of elements in the layout and $k$ the number of properties per element.
Following PolyGen \cite{nash2020polygen}
%, our positional encoding for each token consists of 
we use two additional inputs per token in the sequence:
%use a \textit{positional embedding}\cite{vaswani2017transformers} consisting of
the sequence index $i$ and the type $t_i$ of each value.
%The sequence index generates a learned \textit{positional embedding}\cite{vaswani2017transformers}.
Type $t_i$ is the index of a constraint value inside its constraint tuple and indicates the type of the value (x-location, height, angle, etc.). Finally, we add a special stopping token $s$ as last element of the sequence to indicate the end of the sequence.

\paragraph{Autoregressive Model}
Our element constraint model $f_{\theta}^N$ models the probability of a sequence by its factorization into step-wise conditional probabilities:
\begin{equation}
    p(S_N; \theta) = \prod_{i=1}^{k M_N} p(v_i | v_{<i}; \theta),
\end{equation}
where $\theta$ are the parameters of the model.
Given a partial sequence $v_{<i}$, the model predicts a distribution over values for the next token in the sequence $p(v_i| v_{<i}; \theta) = f_{\theta}^N(v_{<i}, (1 \dots i-1), t_{<i})$, that we can sample to obtain $v_i$. We implement $f_\theta$ with a small version of GPT-2~\cite{radford2019language} that has roughly 10 million parameters. For architecture details, please refer to Section \ref{sec:architecture} and the supplementary material.
%Appendix \ref{app:architecture}.

\paragraph{Coordinate Quantization}
We apply 6-bit quantization for all coordinate values except $\alpha$, which we quantize to 5 bits. We learn a categorical distribution over the discrete constraint values in each step of the model. Nash et al.~\cite{nash2020polygen} have shown that this improves model performance, since it facilitates learning distributions with complex shapes over the constraint values.


% \paragraph{Training Sequence} \wamiq{We consider the origin at the top-left of the image representation of the floorplan. We order our boxes by first sorting them in horizontal direction, and then the vertical direction. The order used in both the sorts is an increasing order. This gives us a list of either $\boxx$ or $tbox$. We have no special token to denote the end of a given box as the individual boxes are represented by fixed-length tuples. The training sequence is thus a list of boxes $\mathbf{B}= (\boxx[1], \boxx[2], \ldots, \boxx[n_b])$, where $n_b$ is the number of boxes. The number of tokens in the sequence depends on the dataset and the type of box-representation, but even our largest sequences have a length of approximately 200, which is small enough to train on a single GPU.}

% \paragraph{Model:} \wamiq{We use a GPT-2 \cite{radford2019language} like architecture as the basis of our model. GPT-2 is a powerful autoregressive model that uses Attention\cite{vaswani2017transformers} to \textit{attend} to every part of the sequence. This is important to us as room placement is significantly affected by rooms that are far away in the spatial domain and with our sorting strategy, the rooms that are far away in space are also far away in the encoded sequence. We use very small models compared to the models in the original paper - the smallest model in the paper has 117 million parameters, while our model has around 10 million parameters.}

\subsection{Edge Model}
\label{sec:edge_model}
We generate relationship edges $R$ between elements that either constrain element parameters or add additional information to the layout. The constraining edges $\mathbf{R}^C$ will be used as constraints during the optimization step, while descriptive edges $\mathbf{R}^D$ add information to the layout and may be needed in down-stream tasks. In floor plans, for example, door and wall edges define walls and doors. We use an autoregressive sequence-to-sequence architecture based on PointerNetworks~\cite{vinyals2015pointer} to generate edges. We train one model for each of the edge types described in Section~\ref{sec:layout_rep}, each models the distribution for one type of edge. All models have the same architecture, but do not share weights.

\paragraph{Sequence Encoding} To flatten the list of edges $R = (N_i, N_j, \rho)$ of any given type $\rho$, we first sort them by the index of the first element $i$, then by the index of the second element $j$.
%
We then concatenate the constraints $N^C_i$, $N^C_j$ corresponding to the elements $N_i, N_j$ in each edge to get a sequence of element constraints. We use a learned embedding $n_j^{\rho} = g_{\phi_{\rho}}(N^C_j)$, giving us a sequence of element embeddings $S_{\rho} = (n_{j_i}^{\rho})_{i=1}^{2 M_{\rho}}$, where $M_{\rho}$ is the number of edges of a given type $\rho$.
%For constraining edges, we instead encode the element constraints $n_j^{\rho} = g_{\phi_{\rho}}(N^C_j)$, since the elements are only available after optimization.
%
Two additional inputs are added for each token: the index $i$ and the type $t_i$, indicating if a token corresponds to the source or target element of the edge. The last token in the sequence is the stopping token $s$.

Due to our ordering, groups of edges that share the same source element $N_i$, are adjacent in the list.
For types of edges where these groups are large, that is, where many edges share the same source element, we can shorten the sequence by including the constraint of a source element only once at the start of the group, and then listing only the constraints of the target elements $N_j$ that are connected to this source element. The end of a group is indicated by a special token $e$. We use this shortened sequence style for the adjacency edges of floor plans.

\paragraph{Autoregressive Model}
Similar to the element constraint model, the probability of an edge sequence $S_{\rho}$ is modeled by a factorization into step-wise conditional probabilities. Unlike the element constraint model, however, the edge model $f_{\phi_{\rho}}^R$ outputs a pointer embedding~\cite{vinyals2015pointer}:
\begin{equation}
    q_i^{\rho} = f_{\phi_{\rho}}^R(n_{j_{<i}}^{\rho}, (1 \dots i-1), t_{<i}).
\end{equation}
We compare this pointer embedding to all element embeddings using a dot-product to get a probability distribution over elements:
\begin{equation}
    p(n_{j_i}^{\rho}{=}n_k^{\rho} | n_{j_{<i}}^{\rho}; \phi_{\rho}) = \mathrm{softmax}_k\left((q_i^{\rho})^T n_k\right)
\end{equation}
that we can sample to get the index of the next element constraint in the sequence.

% \paragraph{Training Sequence} \wamiq{The constraints on boxes can be symmetric or asymmetric and this leads to different types of constraint graphs. As an example, a \door constraint is symmetric which means the graph it generates is undirected. In constrast, an adjacency relation is not symmetric as adjacent boxes touch along different edges - top edge of a box touches the  bottom edge its vertically adjacent box. Thus the adjacency constraint generates a directed graph. In our representation, this distinction is removed and we consider all graphs as directed graphs. To flatten this graph into a sequence, we use the previous sorting strategy of boxes, and list all the neighbours of box 1, then all neighbours of box 2 except 1 and so on. These neighbours are then concatenated in the same order with a special \textit{new box} token between neighbours of different boxes. The sequences thus obtained are again reasonably small with \door sequences being as short as 48 token long for both \rplan and \lifull, with \wall sequences as long as 170 tokens on \lifull and \rplan \wall sequences significantly shorter.}

% \paragraph{Model:} \wamiq{This representation introduces the problem that the number of nodes is now variable but the neighbour index/token that the model predicts must be less than this variable number. We use the idea of Pointer Networks\cite{vinyals2015pointer} similar to Polygen\cite{nash2020polygen} to solve this problem. The model is still based on GPT-2, with an encoder and decoder composed of Attention Blocks.}

% \wamiq{Specifically, we first get the box embeddings $\mathbf{e}_b$, from an \textit{unmasked, non-causal} encoder $E$ operating on the box-sequence $\mathbf{B}$. This block does not need to possess the autoregressive property, and thus with attention can generate embeddings that aggregate information from all parts of the sequence providing global context to the embeddings. The decoder $D$, to embed the edge-sequence just uses the box-embeddings with the tokens of the edge-sequence as an index into the box-mbeddings. The decoder is \textit{masked} to be \textit{causal}.
% TODO: describe the operation mathematically}
% \wamiq{The new model on account of using both an encoder and a decoder is twice as big as the box-model, but still lightweight at only 20 million parameters}

\subsection{Optimizing Layouts}
\label{sec:optimization}

We formulate a Linear Programming problem~\cite{boyd2004convex} that regularizes the layout while satisfying all generated constraints:
\begin{equation}
\begin{aligned}
    \min_{\mathbf{N}} \quad & o(\mathbf{N}) \\
    \textrm{s.t.} \quad & \mathbf{N}^C\ \text{are satisfied and}\\
                        & \mathbf{R}^C\ \text{are satisfied},
\end{aligned}
\end{equation}
where $o(\mathbf{N})$ is a regularization term. In floor plans, for example, we minimize the perimeter of the floor plan $o(\mathbf{N}) = W + H$, where $W$ and $H$ are the width and height of the floor plan's bounding box. This effectively minimizes the size of the layout, while keeping the optimization problem linear. This regularization encourages compactness and a bounded layout size, resulting in layouts without unnecessary gaps and holes. The definition of the constraints depend on the type of layout.

%Appendix~\ref{app:optimization}.

In floor plans, the $x,y,w,h$ parameters of each element are bounded between their maximum and minimum values; we use $[0, 64]$ as bounds in our experiments.
%
Each element constraint $N^C$ adds constraints of the form $v^C (1-\epsilon) \leq v \leq v^C (1+\epsilon)$, for each value $v^C$ in the element constraint $N^C$ and corresponding value $v$ in the element $N$. In our experiments, we set $\epsilon = 0.1$.
%
Horizontal adjacency edges $R = (N_i, N_j, \rho)$ add constraints of the form $x_i + w_i = x_j$, and analogously for vertical adjacency edges.

The layout width $W$ is computed by first topologically sorting the elements in the subgraphs formed by horizontal adjacency edges, and then defining $W \coloneqq x_m + w_m$ for the last (right-most) element $N_m$ in the topological sort. $H$ is computed analogously. Note that we do not define $W \coloneqq \max_i x_i + w_i$ to avoid the additional constraints needed to optimize over the maximum of a set. A detailed list of constraints for furniture layouts is given in the supplementary material. The challenge of designing the optimization is to keep the optimization fast and simple
%(i.e. linear)
and to make it work in conjunction with the neural networks.

% We have a standard parameterization of the \textit{floor-planning} problem\cite{boyd2004convex}. We have $N$ boxes, each of which is parameterized by four (discrete) variables $x_i, y_i, w_i, h_i$, $i \in \{1, \ldots, N\}$, and we seek the optimal $\hat{x_i}, \hat{y_i}, \hat{w_i}, \hat{h_i}$, Additionally, we have two more \textit{global} variables $H$ and $W$, which are the height and the width of the bounding box of the layout.

% Following \cite{boyd2004convex}, we formulate a Linear Programming problem by setting the objective function $\mathcal{L} $ to be the perimeter of the bounding box of the plan $\mathcal{L} = 2(H + W)$. For \textit{floor plans}, we focus on simple adjacency constraints. The pointer networks in Section \ref{} %TODO: add reference to constraint generation
% generate two graphs $\mathcal{H}=(V^H, E^H) $ and $\mathcal{V}=(V^V, E^V)$, where $(e_i, e_j) \in V^H$ means that box $i$ touches $j$ along the left-edge of box $i$. This means we add the constraint $x_i + w_i = x_j$. An edge in $\mathcal{V}$ means a shared edge in the vertical direction. In our generation pipeline, the model \ref{} %TODO get element constraint model
% generates $w_i, h_i$ for all boxes (plus $\tau_i$ which is not used in optimization). With these boxes, we then generate the constraint graphs for them and solve for $x_i, y_i$ for all boxes. Additionally, we also use the generated $w_i, h_i$ as constraints by enforcing an additional constraint that $ \ceil{(1 - \epsilon) w_i} \leq \hat{w_i} \leq \floor{(1 + \epsilon) w_i}$. We use an $\epsilon=0.1$.

% TODO: We describe the dataset later, so does this belong here? As the RPLAN/LIFULL datasets are quantized to 6-bits in the spatial variables, we already know that the bounding box of the layout will be a $64 \times 64$ quad. Thus, any feasible solution returned by our solver is an optimal solution.


\subsection{User-provided Constraints}
\label{sec:user_constraints}

We can condition our models on any user-provided element constraints.
%and the edge model on any user-provided edge constraints.
We add an encoder
%to both of these models,
to both the element constraint model and the edge model,
following the encoder/decoder architecture described in~\cite{vaswani2017transformers}. The
%element constraint
encoder
%$c^E$
takes as input a flattened sequence
%$S_E^C$
of user-provided constraints, enabling cross-attention from the sequence
%$S_E$
that is currently being generated to the list of user constraints.
%$S_E^C$.
Note that the user-provided constraints do not have to represent the same quantities as the output sequence. In floor plans, for example, we can condition both the element constraint model and the edge model on a list of room types, room areas and/or a floor plan boundary.
%Similarly, the adjacency edge models can be conditioned on a list of door edges.
%The encoder/decoder architecture can `translate' these conditions to compatible output sequences.

%In \emph{floor plans}, we flatten a list of \paul{TODO: finish}

% that enables cross-attention to the list of user constraints.

% Could add user-provided constraints directly to set of generated constraints, but there would be no mechanism to encourage the resulting larger set of constraints to be satisfiable.

\subsection{Network Architecture}
\label{sec:architecture}
Our models use the Transformer \cite{vaswani2017transformers} as a building block. Our Element Constraint Model and the Edge model are very similar to the Vertex and Face models from PolyGen \cite{nash2020polygen} in organization. The building block for the Transformers themselves is based on the GPT-2 model, specifically, we use the GELU activation \cite{hendrycks2016gelu}, Layer Norm \cite{layernorm19} and Dropout. For a complete description, please refer to the supplementary.

The model for element constraint generation consists of 12 Transformers blocks. Our sequence lengths depend on the particular dataset used, and are listed in the supplementary.
%
The edge generation model is a Pointer Network with two-parts: 1. An encoder which generates embeddings, and can attend to all elements in the sequence of element constraints and 2. A decoder which generates pointers, and can attend to elements in an autoregressive fashion. In our experiments, we use an encoder with 16 layers and a decoder with 12 layers. 
We use 384 dimensional embeddings in all our models.

\begin{figure}[t]
    \centering
    \includegraphics[height=1.7in]{images/enc_dec_image.pdf}
    \caption{The constrained element generation model. Having an unmasked encoder allows our network to attend to all elements of the constraint sequence.
    %The grey blocks are stacked multiple times.
    }
    \label{fig:enc_dec_model}
\end{figure}

Constrained generation %(see Section \ref{sec:results})
is performed by a variant of the unconstrained models. Concretely, we add a constraint encoder to both the element constraint model and the edge models resulting in an encoder-decoder architecture. In the edge models, we concretely change the encoder of the Pointer Network to an encoder-decoder architecture.
%$\hat{\mathbf{E}}-\hat{\mathbf{D}}$
(Figure \ref{fig:enc_dec_model}).
The constraint encoder
%$\hat{\mathbf{E}}$
is a stack of Transformer blocks allowed to attend all elements of the constraint sequence. The decoder
%$\hat{\mathbf{D}}$
is another stack of blocks allowed to attend to all tokens in the constraint sequence.
%When generating elements themselves, it attends to elements in an autoregressive fashion.
%Additionally, it performs cross-attention with the activations from $\hat{\mathbf{E}}$.
We use 8 layers for constraint encoder in the element model and 3 layers in the edge-model.

\paragraph{Training Setup}
\label{sec:traning_setup}
We implemented our models in Pytorch\cite{paszke2017automatic}. Our models and sequences are small enough so we train on a single NVIDIA-V100 GPU with 32 GB memory. We use the Adam \cite{DBLP:journals/corr/KingmaB14} optimizer, with a constant learning-rate of $10^{-4}$, and linear warmup for 500 iterations. The element generation model is trained for 40 epochs, while the other models are trained for 80 epochs. It takes approximately 6 hours to train for our largest model for constrained generation.

\paragraph{Inference} The inference time depends on the type of sequence being sampled. Our large sequences have about 250 tokens. For this sequence length, generating a batch of 100 element constraint sequences  takes about 10s. Given the element constraint sequence, all types of edges can be sampled in parallel. Edge models are larger and need about 60s for a batch of 100 sequences.

==> source/sections/models.tex <==
% As previously alluded to, our models use the Transformer \cite{vaswani2017transformers} as a building block. Our Element Constraint Model and the Edge model are very similar to the Vertex and Face models from PolyGen \cite{nash2020polygen} in roganization. The building block for the Transformers is based on the GPT-2 model, specifically, we use the GELU activation \cite{hendrycks2016gelu}, Layer Norm \cite{layernorm19} and dropout. For a complete description, please refer to the supplementary.

% The model for element constraint generation consists of 12 layers of our Transformers blocks. The sequence lengths depend on the particular dataset used, and are listed in the supplementary.

% The edge generation model is a Pointer Network with two-parts: 1. An encoder which generates embeddings, and can attend to all elements in the sequence of element constraints and 2. A decoder which generates pointers, and can attend to elements in an autoregressive fashion. In our experiments, use an encoder with 16 layers and a decoder with 12 layers. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{images/enc_dec_image.pdf}
%     \caption{The embedding generation model in the Pointer Network. Having an unmasked encoder allows our network to attend to all elements of the constraint sequence}
%     \label{fig:enc_dec_model}
% \end{figure}

% We perform constrained generation (Section \ref{sec:results}). This is performed by a variant of the edge generation model defined previously. Concretely, we change the encoder of Pointer Network to an encoder-decoder network $\hat{\mathbf{E}}-\hat{\mathbf{D}}$. The encoder $\hat{\mathbf{E}}$ is also a stack of Transformer blocks allowed to attend all elements of the sequence describing the constraints, and the decoder $\hat{\mathbf{D}}$ is another stack of blocks allowed to attend to all elements of the sequence constraints, and also performs cross-attention with the activations from $\hat{\mathbf{E}}$. We use 3 layers for $\hat{\mathbf{E}}$.

% We use 384 dimensional embeddings in all our models.

% \subsection{Training}
% We implemented our models in Pytorch\cite{paszke2017automatic}. Our models and sequences are small enough so we train on a single NVIDIA-V100 GPU with 32 GB memory. We use a constant learning-rate of $10^{-4}$, with a linear warmup for 500 iterations. The element generation model is trained for 40 epochs. The other models are trained for 80 epochs. It takes about 6 hours to train for our largest model for constrained generation.

==> source/sections/related_work.tex <==
%\subsection{Layout Generation}

We will discuss image-based generative models, graph-based generative models, and finally models specialized to layout generation.

% The most straight-forward approach to generating layouts is to convert them to a generic domain in order to apply traditional generative models. In layouts, both the spatial layout of elements and the relationships between elements play an important role, therefore two natural domains to represent layouts are images and graphs. We will discuss approaches specialized to layouts after these two generic domains.
%We will give some examples of image and graph methods that are relevant to layout generation in the following two sections, followed by an overview of generative models that are more specialized to layouts.

\subsection{Image-based Generation}
A straight-forward approach to generate a layout is to represent it as an image and use traditional generative models for image synthesis.
The most promising approach are generative adversarial networks~(GANs)~\cite{Goodfellow2014GANs,Karras2017ProgressiveGrowing,Han18SAG,DBLP:journals/corr/abs-1809-11096,2018arXiv181204948K,SGv2,Karras2020ada}.
Image-to-image translation GANs~\cite{Isola2016Pix2Pix, Zhu2017CycleGAN, NIPS2017_6650, Huang:2018:MUNIT, zhu2019sean,richardson2020encoding} could also be useful for layout generation, e.g., as demonstrated in this project~\cite{chaillou2020archigan}.
Alternatively, modern varitional autoencoder, such as NVAE~\cite{vahdat2020NVAE} or VQ-VAE2~\cite{DBLP:conf/nips/RazaviOV19} are also viable options.
Autoregressive models, e.g.~\cite{Chen2020GPTImage}, also showed great results on larger datasets recently.
When experimenting with image-based GANs, we noticed that they fail to respect the relationships between elements and that they cannot preserve certain shapes (e.g. axis-aligned polygons, sharp corners).

% a task that can be approached with a Conditional GAN~\cite{Isola2016Pix2Pix}, a Cycle GAN~\cite{Zhu2017CycleGAN}, Bicycle GAN~\cite{NIPS2017_6650}, MUNIT~\cite{Huang:2018:MUNIT}, or StyleGAN~\cite{richardson2020encoding}. 
%These GANs have also been adapted to specific applications, such as day-to-night translation~\cite{DBLP:journals/corr/LuanPSB17}, the generation of caricatures~\cite{cao2018cari, richardson2020encoding}, geometric detail synthesis, texture synthesis for building mass models~\cite{KellyGuerreroEtAl_FrankenGAN_SigAsia2018}, and sketch-to-terrain translation~\cite{Guerin:2017:IET} to name only a few. 
%Stanislas Chaillou~\cite{chaillou2020archigan} applies a well-known image translation GAN~\cite{Isola2016Pix2Pix} in a multi-step pipeline to generate floor plans.

% For layout generation, purely image-based methods fail to respect distributions of relationships among layout elements, such as the connectivity between rooms in a floor plan, as we show in Section~\ref{sec:results}. Additionally, parsing these images to obtain layout elements and their relationships is often non-trivial and error-prone. Explicitly generating the relationships between elements as graph edges improves the distribution of element relationships in generated layouts.

\subsection{Graph-based Generation}
In order to capture relationships between elements, various graph-based generative models have been proposed~\cite{Wang:2018:AAAI:graphGAN, Li:2018:LDGG, Simonovsky:2018:GraphVAE, You:2018:GraphRNN, GraphFlows2019, GraphAttention2019, GraphEmbedding2020}.
However, purely graph-based approaches only generate the graph topology, but are missing the spatial embedding. The specialized layout generation algorithms described next often try to combine graph-based and spatial approaches.

%Learning distributions over graphs is challenging due to the high-dimensional nature of the problem, non-local dependencies, cycles in the graphs, and varying connectivity patterns among graph nodes. 
% % 
% One line of work designs different linearization strategies to embed the graph as strings, or more recently, into a latent representation, and then sample graphs from the embedded space. 
% % 
% Deepwalk~\cite{Perozzi:2014:DOL} takes a graph and produces a latent representation as an output, while 
% %. It uses local information obtained from truncated random walks to learn latent representations and was applied to categorizing social network graphs, while 
% Li et al.~\cite{DBLP:journals/corr/LiMSRJ17} utilizes adversarial training to produce dialogues that are indistinguishable from human-generated utterances via a reinforcement framework. 
% %where the generator produces suggested dialogues which are then used via the discriminator to produce a score that is utilized as the reward function for the RL. 
% GraphGAN~\cite{Wang:2018:AAAI:graphGAN} embeds graph nodes into a vector space; then an adversarial setup simultaneously uses a generator to learn the connectivity distribution of nodes and a discriminator to model the probability of edges between pairs of vertices. 
% %
% %In the context of meshes, Litany et al.~\cite{DBLP:journals/corr/abs-1712-00268} use a graph autoencoder to learn a latent space and apply it to mesh completion, 
% %Ben-Hamu et al.~\cite{Ben-Hamu:2018:MGS} propose a new image-like multichart parameterization and then use image-GANs for shape synthesis, while Gao et al.~\cite{Gao:2018:AUS} propose using VAE-cycle GAN for deformation transfer between unpaired meshes. 
% %
% Li et al.~\cite{Li:2018:LDGG} learn generative models over graphs that can encode both structure and attributes. They express probabilistic dependencies over graph nodes and edges, and aim to learn distributions over any arbitrary graph.
% %Theirs is one of the first approaches to move away from vector representations of graphs towards more flexible graph representations. 
% With a similar motivation, 
% GraphVAE~\cite{Simonovsky:2018:GraphVAE} generates discrete graphs by using a decoder to directly output a probabilistic fully-connected graph of a predefined maximum size as a variational autoencoder. In contrast, GraphRNN~\cite{You:2018:GraphRNN} is a deep autoregressive model that progressively learns to generate graphs by decomposing the graph generation process into a sequence of node and edge formations conditioned on the current graph state.


%While generic graph generation methods are well suited to accurately generate relationships between layout elements, in the context of graphical layouts, we work with embedded graphs, i.e. graphs where nodes have some spatial or geometric embedding. Purely graph-based methods have no mechanism to ensure consistency between the generated relationships and the generated embedded elements. We add such a mechanism in the form of an optimization, where element properties are optimized to satisfy the generated edges.

%are able to closely match the target topological feature distributions, generating a final layout by spatially embedding the graph remains a very difficult problem (see Section~\ref{sec:results}). Instead, we use a graph-based method to infer connectivity of the spatial results produced by image-based GANs, and then finally coordinate the results between the spatial and topological domains. 



%The coarsely embedded graphs can be seen as a generalization of sparse point clouds with the graph providing local connectivity information, in contrast to $k$-nearest connectivity utilized in case of learning frameworks proposed for unstructured point clouds~\cite{qi2017pointnet, qi2017pointnet++, guerrero2018pcpnet, wang2018dgcnn}. We also draw on the idea of utilizing a trained latent space for developing a robust GAN-setup for weakly structured data as has been shown in the case of point cloud synthesis~\cite{achlioptas2017learning, achlioptas2018learning}.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{images/overview.pdf}
    \caption{Overview of our layout generation approach. We generate constraints on the parameters of layout elements with a Transformer~\cite{vaswani2017transformers}, and constraints on multiple types of relationships between elements using Pointer Networks~\cite{vinyals2015pointer}. Both element and relationship constraints are used in an optimization to create the final layout.}
    \label{fig:overview}
\end{figure*}

\subsection{Specialized Layout Generation}

Before the rise of deep learning, specialized layout generation approaches have been investigated in numerous domains, including street networks~\cite{Yang:2013:UPL,Peng:2016:CND}, parcels~\cite{bymw_goodLayout_sigg13,Vanegas:2012:PGO}, floor plans~\cite{Wu:2018:MLD}, game levels~\cite{Yeh:2012:SOW}, furniture placements~\cite{Yu:2011:MakeItHome}, furniture and object arrangements~\cite{Fisher:2012:ESO}, and shelves~\cite{Majerowicz:2014:FYS}.
Different approaches have been proposed for layout generation, such as rule-based modeling~\cite{Prusinkiewicz:1990:ABP,Mueller:2006:PMO}, stochastic search ~\cite{Merrell:2011:IFL,Yu:2011:MHA, Yeh:2012:SOW}, or integer programming~\cite{Peng:2014:CLW,Peng:2016:CND,Wu:2018:MLD}, or graphical models~\cite{Merrell:2010:CGR,Fan:2016:APM,Chaudhuri:2011:PRF,Kalogerakis:2012:APM, Fisher:2012:ESO, Yeh:2013:STP}.

In recent years, most of the focus has shifted to applying deep learning to layout generation.
%Several generative methods that are specialized to various types of layouts have been proposed.
%Several approaches place layout elements one-by-one
A popular and effective technique
%is to design a learning framework that
places elements one-by-one, ~\cite{Wang:2018:DCP, LayoutVAE:ICCV:2019, NTG:ICCV:2019}, while a different approach first generates a layout graph and then instantiates elements according to the graph~\cite{IGS:CVPR:2018,PlanIT:2019:Wang,SOA:ICCV:2019}. Both of these approaches are problematic in layouts such as floor plans, that have many constraints between elements, such as zero-gap adjacency and door connectivity.
%are harder to satisfy (no gaps between rooms, satisfying the given connectivity, alignment constraints, etc.).
In such a settings it is non-trivial to a) train a network to generate constraints that admit a solution, and b) find elements that satisfy the constraints in a single forward pass. 
Recently proposed methods~\cite{Wu_DeepLayout_2019, Graph2Plan20, housegan2020} circumvent these problems by requiring manual guidance as input, or by requiring manual post-processing. Due to these requirements, these methods are not fully generative.
%
%assuming satisfiable constraint graphs to be given as input~\cite{Graph2Plan20, housegan2020}. Wu et al.~\cite{Wu_DeepLayout_2019} require only the boundary of the layout as input, but room connectivity needs to be added manually as a post-process. These methods are not fully generative, since they require layout graphs or boundaries as input.
%
%Deep learning has also been used for floor plan reconstruction from images~\cite{Liu:2018:Floornet,DFP:ICCV:2019}.
%
%Wu et al.~\cite{Wu_DeepLayout_2019} require only the outline of the floor plan as input, however room connectivity is added manually as a post-process.
%In our method, we improve upon this work in several ways. First, their inputs are floorplan outlines which means that a lot of complexity is already given; designing the outline first is inconsistent with many architectural workflows. Second, we also generate the connectivity between the rooms. And finally, we can provide arbitrary constraints to the floor plan, ranging a fully generative model with no constraints at all, to large numbers of constraints on room numbers, locations, and sizes, including completion of partial floor plans.
%
Recently, Xu et al. introduced PolyGen~\cite{nash2020polygen}, a method to generate graphs of vertices that form meshes with impressive detail and accuracy.
%This method uses Transformers~\cite{vaswani2017transformers} and Pointer Networks~\cite{vinyals2015pointer} to generate meshes with impressive detail and accuracy.
We base our method on a similar architecture, but generate layout constraints instead of directly generating the final layout. Layout elements are then found in an optimization step based on the generated constraints. This gives us layouts where elements accurately satisfy the constraints.
%This allows us to optimize layout elements in an optimization step that improves constraint satisfaction in the generated layouts.
%based on these constraints in an optimization step that improves constraint satisfaction.
%to condition our generated layout on arbitrary input constraints.


==> source/sections/results.tex <==
We evaluate free generation of layouts, generation constrained by a given boundary, and generation constrained by additional user-provided constraints. We will focus on floor plans in this section. Furniture layouts are evaluated in the supplementary material.
\paragraph{Datasets}
We train and evaluate on two floor plan datasets.
%
The RPLAN dataset~\cite{Wu_DeepLayout_2019} contains 80k floor plans of apartments or residential buildings in an Asian real estate market between 60$\text{m}^2$ to 120$\text{m}^2$.
%The dataset was prefiltered to remove outliers, such as discarding floor plans that have many tiny rooms or few huge rooms, floor plans that are too large or small. 
%
The LIFULL dataset~\cite{lifull} contains 61k floor plans of apartments from the Japanese housing market. The apartments in this dataset tend to be more compact.
%It was originally gathered by Lifull Home's, a real estate and housing information aggregation web service, and is made available for research in cooperation with the Rakuten Institute of Technology.
The original dataset is given as heterogeneous images, but a subset was parsed by Liu et al.~\cite{Liu:2017:RasterToVector} into a vector format.
%
In both datasets we use 1k layouts for each of testing and validation, and the remainder for training.
% \paul{TODO: furniture?}
\paragraph{Baselines}
%We compare with state-of-the-art methods for layout generation.
StyleGAN~\cite{styleGan18} generates a purely image-based representation of a layout. We render the layout into an image to obtain a training set, including doors and walls (see the supplementary material), and parse the generated images to obtain layouts. Graph2Plan~\cite{Graph2Plan20} generates a floor plan given its boundary and a layout graph that describes rough room locations, types, and adjacencies. Door connectivity is generated heuristically. RPLAN~\cite{Wu_DeepLayout_2019} generates a floor plan given its boundary, with a heuristically-generated door connectivity. All baselines are re-trained on each dataset.
\begin{table}[t]
\caption{Free generation of layouts. We compare the FID and layout statistics on two datasets to the state-of-the-art. Note that Graph2Plan uses a ground-truth layout graph as input, and both RPLAN and Graph2Plan use the ground truth boundary as input. We evaluate both free generation with our method and conditional generation. Our method improves upon the baselines with less input guidance.}
\centering 
% \small
\footnotesize
\setlength{\tabcolsep}{5pt}
\begin{tabular}{@{}llS[table-format=2.2]S[table-format=2.2]S[table-format=2.2]S[table-format=2.2]S[table-format=2.2]c@{}} 
% \begin{tabular}{@{}llccccc@{}} 
\toprule
dataset & method & {FID} & $\hat{s}_{t}$ & $\hat{s}_{r}$ & $\hat{s}_{a}$ & $\hat{\mathbf{s}}_\textbf{avg}$ \\
\midrule \midrule
\multirow{4}{*}{RPLAN}
& StyleGAN. & 25.29 & 46.74 & 4.41 & 7.85 & 19.67 & \\
& Graph2Plan & 29.26 & 0.83 & 5.63 & 18.93 & 8.46 & \\
& RPLAN & \boldentry{21.29} & 5.38 & 1.53 & 4.38 & 3.76 & \\
& ours free & 21.47 & 1.00 & 1.00 & \boldentry{1.00} & \boldentry{1.00} & \\
& ours cond. & 27.27 & \boldentry{0.81} & \boldentry{0.94} & 1.34 & 1.03 & \\
\midrule
\multirow{4}{*}{LIFULL}
& StyleGAN & 28.06 & 44.54 & 2.32 & 1.96 & 16.27 & \\
& Graph2Plan & 29.50 & 9.21 & 0.94 & 1.37 & 3.84 & \\
& RPLAN & 32.98 & 40.54 & 2.02 & 4.10 & 15.55 & \\
& ours free & \boldentry{26.15} & 1.00 & 1.00 & 1.00 & \boldentry{1.00} & \\
& ours cond. & 31.94 & 5.70 & \boldentry{0.71} & \boldentry{0.50} & 2.30 & \\
\bottomrule
\end{tabular}

\label{tab:free_generation}
\end{table}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{images/free_generation.pdf}
    \caption{Free generation of floor plans. We compare our method to three baselines. Rooms are colored by room type, with an overlaid door connectivity graph. Nodes on the graph have icons based on the room type. Our three-step approach improves upon the room layout and connectivity compared to previous approaches, while requiring less guidance as input.}
    \label{fig:free_generation}
\end{figure*}
\paragraph{Metrics} We compare generated layouts to ground truth layouts using two metrics: The \emph{Fr\'echet Inception Distance} (FID)~\cite{heusel2017gans} computed on rendered layouts, and a metric based on a set of \emph{layout statistics} that measure layout properties that the image-based FID is less suitable for. Layout statistics are grouped into topological statistics $S_t$ such as the average graph distance in the layout graph between any two element types,
%(in floor plans: how many doors separate two rooms),
element shape statistics $S_r$ such as the aspect ratio or area, and alignment statistics $S_a$ such as the gap between adjacent elements, or their boundary alignment. We believe that our proposed statistics are more useful to evaluate layouts than FID. FID is more suitable to evaluate generative models trained on natural images, but we show the FID metric for completeness as it is more widely used.
%(see the supplementary material for details).

{\em Topological statistics} $S_t$ are specialized to measure the topology of a layout graph~\cite{bookStreet,Tarabishy2019DeepLS}:
\begin{itemize}[itemsep=-3pt]
    \small
    \item[$s_t^r$:] the average number of elements of a given type in a layout.
    \item[$s_t^h$:] a histogram over the number of elements of a given type in a layout.
    \item[$s_t^t$:] the number of connections between elements of type $a$ and elements of type $b$ in a layout.
    \item[$s_t^d$:] the average graph distance between elements of type $a$ and elements of type $b$ in a layout.
    \item[$s_t^e$:] a histogram of the graph distance from an element of type $a$ to the exterior.
    \item[$s_t^c$:] a histogram of the degree of an element of type $a$, i.e. how many connections the element has to other elements.
    \item[$s_t^u$:] The number of inaccessible elements of type $a$ in a layout.
\end{itemize}
{\em Element shape statistics} $S_r$ measure simple properties of the element bounding boxes:
\begin{itemize}[itemsep=-3pt]
    \small
    \item[$s_r^c$:] a histogram of location distributions for each element type.
    \item[$s_r^a$:] a histogram of area distributions for each element type.
    \item[$s_r^s$:] a histogram of aspect ratio distributions for each element type.
\end{itemize}
{\em Alignment statistics} $S_a$ measure alignment between all pairs of elements:
\begin{itemize}[itemsep=-3pt]
    \small
    \item[$s_a^c$:] a histogram of the distances between element centers, separately in x and y direction.
    \item[$s_a^g$:] a histogram of the gap size distribution between element bounding boxes (negatives values for overlaps).
    \item[$s_a^a$:] a histogram of the distances between element centers along the best-aligned (x or y) axis.
    \item[$s_a^s$:] a histogram of the distances between the best-aligned sides of the element bounding boxes.
\end{itemize}
The same alignment statistics are also computed between pairs of elements that are connected by descriptive edges.

We average each statistic over all layouts in a dataset and compare the resulting averages $\overline{s}$ to the statistics of the test set. We use the Earth Mover's distance~\cite{Rubner:1998:MDA} to compare histograms:
\begin{equation}
\hat{s}_{*} = \frac{1}{|S_*|}\sum_{s \in S_*}\frac{\text{EMD}(\overline{s}, \overline{s}^\text{gt})}{\text{EMD}(\overline{s}^\text{ours}, \overline{s}^\text{gt})},
\end{equation}
where $\overline{s}^\text{ours}$ and $\overline{s}^\text{gt}$ are the average statistics of our and ground truth distributions, and $*$ can be $t$, $r$ or $a$. The average over all $\hat{s}_{*}$ is denoted $\hat{\mathbf{s}}_\textbf{avg}$.
Non-histogram statistics use the L2 distance instead of the EMD.
%We take an average over element types $a$ and $b$, weighted by the relative occurrence frequency of the elements, to get a single distance value for each statistic.

%We compute the Earth Mover's Distance~\cite{Leving:2001:EMD} (EMD) between distributions $s$ of generated and ground truth layouts, normalize value ranges by computing statistics relative to our method, and average over each group:
%$\hat{s}_{*} = \frac{1}{|S_*|}\sum_{s \in S_*}\frac{\text{EMD}(s, s^\text{gt})}{\text{EMD}(s^\text{ours}, s^\text{gt})}$, where $s^\text{ours}$ and $s^\text{gt}$ are our and ground truth distributions, and $*$ can be $t$, $r$ or $a$. The average over all $\hat{s}_{*}$ is denoted $\hat{\mathbf{s}}_\textbf{avg}$.

\paragraph{Free Generation} In a first experiment, we generate floor plans fully automatically, without any user input, by sampling the distribution learned by our constraint model.
%We compare all baselines to two versions of our method: the standard version with optimization and a version without optimization, where all element parameters are generated directly.
A comparison to all baselines is shown in Table~\ref{tab:free_generation} and Figure~\ref{fig:free_generation}. Note that among the baselines, only StyleGAN can generate floor plans without user input, while Graph2Plan and RPLAN need important parts of the ground truth as input. For example, we sample topologies and boundaries from the ground truth and give them to the other methods as input. This gives other methods a significant advantage in this comparison. The FID score correlates most strongly with the adjacency statistics, since adjacencies can be captured by only considering small spatial neighborhoods around corners and walls of a floor plan, but does not capture topology or room shape statics accurately that require considering larger-scale features. Unsurprisingly, StyleGAN performs reasonably well on the FID score and adjacency statistics, but shows a poor performance on topological statistics which are mainly based on larger-scale combinatorial features of the floor plans.
%The topological statistics $\hat{s}_t$ are mainly based on larger-scale combinatorial features of the floor plans, making a traditional image-based method like StyleGAN less suitable to accurately capture them.
Graph2Plan receives the topology as input giving it a good performance in topological statistics, but it struggles with room alignment. The RPLAN baseline is specialized to the RPLAN dataset, as shown in the large performance gap between RPLAN and LIFULL. In summary, our proposed framework improves significantly on the state-of-the art, in terms of layout topology, element shape, and element alignment, even though RPLAN and Graph2Plan received significant help from ground truth data.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{images/boundary_gen.pdf}
    \caption{Boundary-constrained generation. Left: input boundary constraint; right: floorplans generated with this constraint.}
    \label{fig:boundary_conditioned_generation}
\end{figure*}
\paragraph{Boundary-constrained Generation} As described in Section~\ref{sec:user_constraints}, we can condition both our element constraint model and our edge model on input constraints provided by the user. Here, we show floor plan generation constrained by an exterior floor plan boundary given by the user. We parse the exterior of the given boundary into a sequence of rectangular elements that we use as input sequence for the encoders of our models. At training time, we use the exterior of ground truth floor plans as input. This trains the models to output sequences of element constraints and edges that are roughly compatible with the given boundary. In the optimization step, we add non-overlap constraints between the generated boxes and the given boundary. Additionally, since the interior boxes are generated in sequence from left to right, we can initialize the first generated box to match the left-most part of the interior area. Figure~\ref{fig:boundary_conditioned_generation} show multiple examples of floor plans that were generated for the boundary given on the left. Quantitative results obtained by conditioning on all boundaries in the test set are provided in the last row for each dataset in Table~\ref{tab:free_generation}. The boundary-constrained floor plans show slightly lower performance in the average layout statistics and FID scores, but still perform much better than RPLAN, which also receives the boundary as input. We can see that our approach gives realistic floor plans that satisfy the given boundary constraint.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/room_conditioned_generation.pdf}
    \caption{Element-constrained generation. Left: The type, width, and height of the these rooms are used as input constraints. Right: example layouts generated with these constraints. Note that the elements form regions of the same types and approximately the same width and height as the room constraints.}
    \label{fig:room_constrained_generation}
\end{figure}
\paragraph{Element-constrained Generation} Our approach can also handle constraints that are given in a different format than the output. We constrain our model to produce a given set of room types, widths, and heights. Results are shown in Figure~\ref{fig:room_constrained_generation}. Even though these constraints are quite limiting, our model produces a large variety of results, while still approximately satisfying the given constraints. 
\paragraph{Discussion}
Our work also has some limitations. For example, the constraint generation network can generate invalid constraints between elements, e.g. doors between rooms that do not share a wall. We can easily identify and remove these constraints. In addition, some constraints result in optimization problems that are infeasible. We simply ignore such samples. Further, like other methods, our work generates a small percentage of low quality results, however, not nearly as many as other methods, which is reflected in the statistics. 

%Both of our versions have a similar performance, showing that our two-step autoregressive architecture is well suited for layout generation. In the next section, we show that our optimization step is necessary to handle user constraints.

%, limiting the number of samples these methods can produce.

% \subsubsection{Furniture}
% conditioned on door and room box
% \begin{itemize}
%     \item (Quant. comparison with StyleGAN using Statistics?) - if we have time to generate some furniture layouts with StyleGAN
%     \item (Quant. comparison with StyleGAN using FID score?) - if we have time to generate some furniture layouts with StyleGAN
%     \item (Qual. comparison with StyleGAN image-only method?)- if we have time to generate some furniture layouts with StyleGAN
%     \item Qualitative examples
% \end{itemize}

% \subsection{Conditional Generation}

% \paragraph{Metrics}
% Same as for free generation before plus how well we satisfy the condition/constraints given by the user

% \subsubsection{Floor Plans}
% conditioned on various user constraints
% \begin{itemize}
%     \item Quant. Comparison with 5-tuples and RPLAN  using Statistics
%     \item Quant. Comparison with 5-tuples and RPLAN using FID score
%     \item Qual. comparison with 5-tuples and RPLAN
% \end{itemize}

% \subsubsection{Furniture}
% conditioned on door and room box + various user constraints
% \begin{itemize}
%     \item (Quant. comparison with StyleGAN using Statistics?) - if we have time to generate some furniture layouts with StyleGAN
%     \item (Quant. comparison with StyleGAN using FID score?) - if we have time to generate some furniture layouts with StyleGAN
%     \item (Qual. comparison with StyleGAN image-only method?)- if we have time to generate some furniture layouts with StyleGAN
%     \item Qualitative examples
% \end{itemize}

% \subsubsection{Furnished Floorplans}
% Just qualitative results

